Using Monocular Vision and Human Body Priors for AUVs to Autonomously Approach Divers

Direct communication between humans and autonomous underwater vehicles (AUVs) is a relatively underexplored area in human-robot interaction (HRI) research, although many tasks (\eg surveillance, inspection, and search-and-rescue) require close diver-robot collaboration. Many core functionalities in this domain are in need of further study to improve robotic capabilities for ease of interaction. One of these is the challenge of autonomous robots approaching and positioning themselves relative to divers to initiate and facilitate interactions. Suboptimal AUV positioning can lead to poor quality interaction and lead to excessive cognitive and physical load for divers. In this paper, we introduce a novel method for AUVs to autonomously navigate and achieve diver-relative positioning to begin interaction. Our method is based only on monocular vision, requires no global localization, and is computationally efficient. We present our algorithm along with an implementation of said algorithm on board both a simulated and physical AUV, performing extensive evaluations in the form of closed-water tests in a controlled pool. Analysis of our results show that the proposed monocular vision-based algorithm performs reliably and efficiently operating entirely on-board the AUV.

==> X_oldfiles/Unused_results.tex <==
\section{RESULTS}
\label{sec:results}
We tested a total of 54 cases with various 


\input{fig/aggregate_trial_data}

% \begin{figure}[H]
%     \centering
%     \scalebox{0.2}{\input{fig/jiyeon_success_big.pgf}}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \scalebox{0.2}{\input{fig/mike_fail_big.pgf}}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \scalebox{0.2}{\input{fig/jiyeon_success_big.pgf}}
         \caption{Success example with narrow shoulder width diver ($35cm$), long distance ($9m$), and turned-away angle($90^{\circ}$)}
         \label{fig:success}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \scalebox{0.2}{\input{fig/mike_fail_big.pgf}}
         \caption{Failure example with wide shoulder width diver ($45cm$), long distance ($9m$), and head-on angle($0^{\circ}$)}
         \label{fig:fail}
     \end{subfigure}
        \caption{\ref{fig:success}: LoCO was turned away from a diver at the beginning. Through the SEARCH and APPROACH states, LoCO detected the diver and placed itself at the designed distance from the diver, \ref{fig:fail}: LoCO was facing a diver and started with the APPROACH state. However, it kept losing the diver because PD from bounding box (spikes in the PD error) caused unstable overshoot to ADROC.}
        \label{fig:errors}
\end{figure}

==> fig/aoc_components.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/aoc_components.jpg}
    \caption{Software components of the DR-AOC algorithm.}
    \label{fig:aoc_components}
    \vspace{-6mm}
\end{figure}

==> fig/aoc_statemachine.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/aoc_statemachine.jpg}
    \caption{Detail on the  DR-AOC state machine, which manages the overal status of the algorithm's operation.}
    \label{fig:aoc_statemachine}
    \vspace{-6mm}
\end{figure}

==> src/acknowledgments.tex <==
\section*{ACKNOWLEDGEMENTS}
The authors wish to thank their families, research collaborators, trial participants, and funding partners, in particular: Sophie Fulton, Jiyeon Hwang, Md Jahidul Islam, Spencer Ludlam, August Walter, the LoCO AUV team, the National Science Foundation,  and the Minnesota Robotics Institute.

==> src/graveyard.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OLD RLEATED WORK
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Visual Object Tracking}
% \label{sec:related:tracking}
% A number of works have addressed the topic of visual object tracking in the underwater domain.
% For example, Katijia et al.~\cite{katija2021visual} presented stereo-camera-based detection and tracking methods with Machine Learning-Integrated Tracking algorithms for tracking underwater animals. 
% However, their method uses a workstation GPU on a mothership via a tether rather than hardware onboard the AUV.
% This is not realistic for tetherless AUVs, which are often equipped with mobile GPUs (which are less computationally powerful than a workstation GPU) or only a CPU.

% Human detectors/trackers typically output bounding boxes and body joints (body pose estimation)~\cite{nguyen2016human}. 
% Shkurti et al.~\cite{8206280} proposed a deep learning-based approach, Recurrent ReducedYOLO, which allows AUVs to track objects using a camera and follow them using the ratio between a bounding box area and a total image area instead of explicit distance estimation. 
% However, this approach struggles when an object can result in different-sized bounding boxes from the same distance.
% In this paper, we propose using diver body pose estimation in addition to bounding box detections to estimate the relative distance between the diver and AUV.
% Pose estimation with a monocular camera has become popular due to its potential applications and higher accuracy compared with bounding box detection~\cite{chen2020monocular}. 
% Diver body pose estimation has previously been utilized for estimating the relative 3D pose between two AUVs~\cite{islam_robottorobot_2020}.
% However, this method runs slowly (2$fps$) and deals with robot-to-robot relative pose estimation instead of estimation of the relative pose between an AUV and a diver, as in our work.
% While body pose estimation is more accurate than simple bounding box detections, its accuracy suffers significantly from occlusion of any body part. 
% Bounding box detections are more tolerant than body pose estimations to occlusion cases, which leads us to use the two to complement each other.

% \subsection{Underwater Human-Robot Interaction }
% \label{sec:related:uhri}
% %Autonomous underwater vehicles (AUVs) face a wide variety of challenges in their operation as previously mentioned, which extend to HRI.
% %Many simple techniques which are common practice in terrestrial HRI require more creative methods underwater due to the nature of the environment.
% Recent years have seen significant advances in underwater human-robot interaction research.
% Work establishing methods for human-to-robot communication for AUVs have focused on using fiducial markers~\cite{dudek_visuallanguagerobot_2007}, hand gestures~\cite{chavez_robustgesturebased_2018, islam_gestures_2019}, and purpose-built control devices~\cite{verzijlenberg_swimmingrobotshuman_2010}.
% The inverse problem of robot-to-human communication has been approached using lights~\cite{demarco_underwaterhumanrobot_2014}, robot motion~\cite{fulton_robotcommunicationvia_2019, demarco_underwaterhumanrobot_2014}, and digital displays~\cite{chavez_caddyunderwaterstereo_2018}.
% Meanwhile, other works have focused on improving the overall communication loop in terms of safety and certainty~\cite{sattar_ensuringsafetyhuman_2014}.
% The majority of related underwater HRI work, however, is concerned with the problem of diver following~\cite{sattar_tracking_2007, islam_2018_toward}.
% Along with these works, there is the more generalized diver-relative navigation proposed by Nad et al.~\cite{nad_diver_tracking_2020}.
% %Our problem we consider is related to these HRI topics (particularly diver following), but is a somewhat different scenario.
% In contrast to diver following or diver relative-navigation, we focus on the problem of an AUV approaching a diver to begin interactions, with no prior knowledge of the situation and only a limited set of sensors.
% Rather than a human seeking to guide our robot to a new place, our robot attempts to guide itself to the human in question, even searching for them if need be.
% While this scenario is inextricably linked to the other HRI topics we have mentioned, our particular set of constraints and requirements, along with our use of monocular vision and diver body pose estimation, differentiate our work.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%FROM OLD EXPERIMENTATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%It consists of two enclosures arranged to the left and right of the central pitch thruster. Each enclosure contains a camera connected to a computer: a Rasberry Pi 4 and Nvidia Jetson TX2 respectively. We only use the right camera connected to the TX2 for our experimental setup.
%Both the diver detection and pose estimation networks were simultaneously running on the TX2, while the Raspberry Pi in the left enclosure provided thruster control based on inference results from the TX2.
%No computation was done off-board, though the AUV was connected to a base station laptop for ease of observation and data collection.

% \subsection{Simulation}
% \label{sec:experiments:simulation}
% The COVID-19 outbreak caused a shortage of manpower and opportunities for field trials to validate the proposed algorithms. 
% To overcome this, we used a LoCO simulation in ROS Gazebo~\cite{koenig_gazebo_2004} as the main tool for developing the algorithms and evaluating them. 
% Particularly, fine-tuning the pseudo distance (Eq~\ref{eq:pd}) and the approach controller in the simulation helped to increase the accuracy of our proposed system and integrate sub-algorithms (Fig. \ref{fig:gazebo}). 
% During our simulations, we observed that the PD based on the pose estimation was invariant to the pose of the diver while the PD based on the diver detection could vary from the same distances. 
% For example, a diver with an extended arm will produce larger-sized bounding box sizes than a diver without, regardless of the distance from the camera. 
% Although the PD based on diver detections is less accurate, it is used as a backup when we have no pose estimation.

==> tab/variables.tex <==
\begin{table}%[H]
    \centering
    \caption{Variables}
    \label{tab:var}
    \begin{tabular}{l}
        Name  \\ \hline
        CMOS sensor size ($mm$)  \\
         focal length ($mm$)  \\
          image size ($pixel$) \\ \hline
    \end{tabular}
\end{table}


% we use the specifications of our mono camera (CMOS sensor size ($mm$) and focal length ($mm$)), image information (image size ($pixel$) and shoulder width of diver ($pixel$)), and shoulder width metric (shoulder size ($mm$)) to design PD. The steps are as follows.
